TRACER: Trajectory-Aligned Learning for Multi-Turn User Simulation

Faithful user simulation is fundamental to building, evaluating, and improving interactive AI at scale. Yet current simulators often produce plausible individual responses without reproducing the intent evolution and outcomes observed in real interactions. We propose TRACER, a multi-turn user simulator that models evolving user intent and aligns simulated trajectories with real ones. TRACER is trained in two stages: supervised fine-tuning on real user dialogues, followed by multi-turn reinforcement learning. The RL stage combines hierarchical outcome- and trajectory-level rewards with deviation-aware advantage modulation, jointly addressing reward sparsity and credit assignment challenges in long dialogues. On real customer-service sessions organized into reference cohorts, TRACER-7B surpasses the strongest baseline by 11.4 conversion F1 points, while outperforming all baselines on group-level conversion-rate error and semantic trajectory distance and generalizing to out-of-distribution scenarios. In human Turing tests, annotators identified TRACER conversations at near-chance accuracy. Building on this simulator, we further introduce the Dynamic Marketing Benchmark, which jointly evaluates persuasion and response quality via simulated interactions, revealing that higher response quality does not necessarily correspond to higher conversion rates.

==> latex/1_intro_old.tex <==
\section{Introduction}
\label{src:intro}
% 【第1段：为什么要有用户模拟器】
% 随着大语言模型在对话系统中的广泛应用，如何高效、可控地获取高质量用户反馈成为推动模型迭代与评估的关键问题。相比于昂贵且不可扩展的人工标注，利用模型构建用户模拟器（user simulator）以生成交互反馈，已逐渐成为一种重要范式【hu2023unlocking】【abbasiantaeb2024let】【qiu2024interactive】。用户模拟器不仅能够用于离线评估对话系统性能，还可以在强化学习或自博弈框架中持续提供训练信号【wu2025collabllm】【wang2025rlver】，从而显著提升系统的交互能力。在实际应用中，这类模拟器已被用于多种场景，例如任务导向对话中的策略优化【davidson2023user】【sekulic2024reliable】【algherairy2025prompting】、推荐系统中的用户响应建模【wang2025user】【zhang2025llm】【zhu2025llm】等。
With the widespread application of Large Language Models (LLMs) in dialogue systems, scalable acquisition of high-quality user feedback has become crucial for model evaluation and improvement. Compared to expensive and non-scalable human annotation, building user simulators with models to generate interactive feedback has gradually emerged as an important paradigm~\citep{hu2023unlocking, abbasiantaeb2024let, qiu2024interactive,dou-etal-2025-simulatorarena}. They support offline evaluation and provide training signals for reinforcement learning or self-play~\citep{wu2025collabllm, wang2025rlver,qian2025userrl}, thereby significantly enhancing the interactive capabilities of the systems. In practice, such simulators have been deployed across diverse scenarios, including policy optimization in task-oriented dialogues~\citep{davidson2023user, sekulic2024reliable,algherairy2025prompting} and user response modeling in recommender systems~\citep{wang2025user, zhang2025llm, zhu2025llm}.

% 【第2段：现有用户模拟器的问题】
% 尽管用户模拟器的研究已受到越来越多关注，现有方法仍然存在明显局限。主流方法通常停留在学习用户的语言风格或用户画像一致性，在建模上将用户profile作为条件输入，引导大语言模型生成符合设定风格的响应【wang2025know】【shi2025you】【ye2025cpoaddressingrewardambiguity】。这类方法在一定程度上能够提高模拟对话的多样性与可控性，但其关注重点仍主要停留在表层语言风格与静态画像约束上，缺乏对真实交互中行为一致性与决策机制的显式建模。其次，在真实多轮对话场景下，真实用户行为不仅取决于静态属性，还受到历史交互、当前情境以及潜在决策状态的共同影响。然而，现有方法中相当一部分在训练范式上仍主要采用面向单轮响应的强化学习优化，而缺乏对完整多轮交互过程的联合建模与优化【wang2025raiden】【liao2025moa】【zhang2026userlm】【wu2026humanlm】。这使得模型虽然能够在局部轮次上生成看似合理的回复，却难以学习真实用户在持续交互中的状态演化、决策连贯性与节奏控制，从而难以真实还原多轮场景下的行为轨迹。受上述限制，现有方法生成的用户反馈在多轮场景中往往容易出现行为不稳定、决策不一致以及场景依赖性不足等问题，从而限制了其在高可信评估与训练中的应用价值。 
%先说是什么
However, existing user simulators still suffer from two fundamental limitations. \emph{(L1) Alignment is limited to linguistic style, not decision-making.} Mainstream methods condition LLMs on static user profiles to elicit persona-consistent responses~\citep{wang2025know,shi2025you,ye2025cpoaddressingrewardambiguity,kim2025few}, aligning simulators with real users only at the surface linguistic level while leaving the underlying decision-making process unaligned, although real multi-turn behavior is jointly driven by interaction history, context, and decision states. \emph{(L2) Optimization is single-turn, not trajectory-level.} Recent methods adopt optimization paradigms tailored to turn-level responses~\citep{wang2025raiden,liao2025moa,zhang2026userlm,wu2026humanlm,dou-etal-2025-simulatorarena}, and thus inherently struggle with reward sparsity and credit assignment in multi-turn interactions, failing to capture state evolution and decision coherence across turns. Consequently, simulated feedback often exhibits behavioral instability and inconsistent decision-making, limiting its utility for high-fidelity evaluation and training.

%Although research on user simulators has attracted increasing attention, existing methods still suffer from clear limitations. Mainstream approaches typically treat the user profile as a conditional input to guide large language models in generating persona-consistent responses~\citep{wang2025know,shi2025you,ye2025cpoaddressingrewardambiguity,kim2025few}.While such methods can improve the diversity and controllability of simulated dialogue to some extent, their primary focus is still limited to surface-level linguistic style and static profile constraints, lacking explicit modeling of behavioral consistency and decision-making mechanisms in real interactions. Furthermore, in real-world multi-turn dialogue settings, user behavior is determined not only by static attributes, but also by the combined influence of interaction history, current context, and latent decision states. However, a considerable portion of existing methods still relies on reinforcement learning paradigms designed mainly for single-turn response optimization~\citep{wang2025raiden,liao2025moa,zhang2026userlm,wu2026humanlm}, without jointly modeling and optimizing the complete multi-turn interaction process.As a result, although these models can produce reasonable single-turn responses, they struggle to capture state evolution, decision coherence, and pacing in sustained interactions, making it difficult to faithfully reproduce multi-turn behavioral trajectories. The resulting user feedback frequently exhibits behavioral instability, inconsistent decision-making, and insufficient contextual  sensitivity, ultimately undermining its utility for high-fidelity evaluation and training.


% 【第3段：我们的工作】
% To this end，我们提出了一种基于真实用户交互数据训练的多轮用户模拟器框架，名为xxx。我们从语言风格一致性与行为一致性两个层面出发，设计了一个两阶段训练方法，以更全面地对齐真实用户分布。不同于仅关注文本风格的建模，我们进一步关注用户在具体任务场景中的行为表达，并为此在用户模拟过程中引入潜在意图状态，以刻画用户在多轮交互中的内在决策倾向以及演化过程。在第一阶段，我们利用真实用户对话数据进行有监督微调，使模型学习细粒度的语言表达模式、上下文依赖的响应习惯以及交互过程中较为粗粒度的意图状态倾向。在此基础上，我们在第二阶段引入多轮对话强化学习，以优化模型在交互层面的行为一致性。具体而言，我们首先设计了分层奖励函数，从结果层与过程层共同约束模拟轨迹与真实轨迹的一致性与合理性。此外，我们发现，在多轮对话中将 session 级反馈简单均匀地分配到各轮，会引入明显的信用分配偏差，从而削弱关键决策步骤的学习效果。因此，我们进一步提出了一种针对多轮交互的优势分配方法（XXX），以更合理地刻画不同轮次对最终行为一致性的贡献。
To address these two limitations jointly, we propose \textbf{TR}ajectory-\textbf{A}ligned \textbf{C}redit Assignment for Us\textbf{ER} Simulation (\textbf{TRACER}), a multi-turn user simulator framework trained on real user dialogues along two complementary axes: linguistic-style consistency, which we treat as a necessary foundation, and session-level behavioral consistency as the central objective. To capture the latter, we further introduce intent states into the simulation process to characterize users' underlying decision tendencies and their evolution across multi-turn interactions. TRACER is trained via a two-stage paradigm that progressively aligns the simulator from linguistic surface to decision-level behavior.
\textbf{Stage 1: Linguistic grounding and intent-state initialization via SFT.} We fine-tune the model on real user dialogues to capture user-like linguistic style and initialize intent states inferred from observed actions.
\textbf{Stage 2: Behavioral alignment via trajectory-level reinforcement learning.} Since SFT only fits per-turn distributions, we introduce RL over multi-turn trajectories to enforce coherent intent evolution and decision-making across turns, jointly closing the decision-level gap of purely linguistic alignment (L1) and the cross-turn incoherence of single-turn RL (L2).
Two key challenges arise: \textbf{(i) Reward granularity}: single outcome-level signal is too coarse to guide intermediate decisions. We address this with a hierarchical reward balancing outcome fidelity and trajectory alignment. \textbf{(ii) Credit assignment}: uniform session-level feedback dilutes learning signals on the few turns actually shaped the outcome. We address this with a trajectory-aligned advantage modulation by its estimated contribution to session-level consistency.
%Two challenges arise. First, a single outcome-level signal is too coarse to supervise intermediate decisions; we therefore design a hierarchical reward that jointly constrains the consistency and plausibility of simulated trajectories against real ones from both the outcome level and the process level (e.g., per-turn alignment over the intent states initialized in Stage 1). 
%Two challenges arise: (i) a single outcome-level reward is too coarse to guide intermediate decisions, for which we design a hierarchical reward that jointly constrains outcome fidelity and trajectory cost against real sessions; and (ii) uniformly broadcasting session-level feedback biases credit assignment on pivotal turns, for which we propose a trajectory-aligned advantage modulation that re-weights each turn by its contribution to session-level consistency.
%Second, naively distributing session-level feedback uniformly across all turns introduces substantial credit-assignment bias, since not all turns are equally decisive, which weakens learning on critical decision-making steps. We thus propose a trajectory-aligned advantage allocation for multi-turn interaction, which re-weights each turn according to its contribution to the final behavioral consistency.
%This stage provides both a faithful linguistic substrate and a warm-started intent prior for the subsequent behavioral optimization.
%From the two complementary perspectives of linguistic style consistency and behavioral consistency, we design a two-stage training paradigm to more comprehensively align the model with the distribution of real users. 
%Unlike prior approaches that focus primarily on textual style, we further emphasize users' behavioral expressions in concrete task scenarios. To this end, we introduce latent intent states into the user simulation process to characterize users' underlying decision tendencies and their evolution throughout multi-turn interactions. In the first stage, we conduct supervised fine-tuning on real user dialogue data, enabling the model to learn fine-grained linguistic expression patterns, context-dependent response habits, and coarse-grained intent state tendencies during interaction. On this basis, in the second stage, we introduce reinforcement learning over multi-turn dialogues to optimize the model's behavioral consistency at the interaction level. Specifically, we first design a hierarchical reward function to jointly constrain the consistency and plausibility of simulated trajectories with respect to real trajectories from both the outcome level and the process level. In addition, we observe that in multi-turn dialogue, simply distributing session-level feedback uniformly across all turns introduces substantial credit assignment bias, thereby weakening learning on critical decision-making steps. Therefore, we further propose an advantage allocation method for multi-turn interaction, to more appropriately characterize the contribution of different turns to final behavioral consistency.

% 【第4段：数据集和结果】
% 为证明我们方法的有效性，我们引入了基于真实用户交互数据的评估基准。该基准涵盖多种真实场景下的多轮对话，并从语言风格一致性、行为一致性等进行评估。实验结果表明，我们的方法在多个指标上显著优于现有用户模拟器方法，尤其在长对话中的行为对齐能力方面取得了明显提升。进一步分析表明，引入轨迹级奖励与改进的优势分配策略对于提升训练稳定性与模拟真实性均具有关键作用。
%To demonstrate the effectiveness of our method, we introduce an evaluation benchmark based on real user interaction data. This benchmark encompasses multi-turn dialogues across diverse real-world scenarios and evaluates from perspectives such as linguistic style consistency and behavioral consistency. Experimental results show that our method significantly outperforms existing user simulator approaches across multiple metrics, achieving particularly notable improvements in behavioral alignment capabilities within long dialogues. Further analysis reveals that the introduction of trajectory-level rewards and the improved advantage allocation strategy play crucial roles in enhancing both training stability and simulation fidelity.
%To demonstrate the effectiveness of our method, we construct a evaluation benchmark comprising over 9,000 real-world customer service dialogues spanning healthcare, automotive, education, and legal domains, and evaluate simulators along three complementary dimensions: session-level behavior, dialogue structure, and semantic consistency. Experimental results show that our method achieves an F1 of 86.2, surpassing the strongest baseline by over 20 absolute points, while simultaneously attaining the best dialogue structure and semantic fidelity scores. A key insight from our evaluation is that \textbf{stylistic alignment alone does not guarantee decision-level behavioral consistency}: role-playing models may match aggregate conversion rates through error cancellation, yet fail to convert the right users. Furthermore, a human-centered Turing test shows that our simulator reaches 49.5\% identification accuracy—converging to the random-guess threshold—whereas even frontier LLMs are detected in over 98\% of cases. Ablation studies confirm that each component—reinforcement learning, trajectory-level reward, and advantage-weighted credit assignment—contributes complementary gains, and that these improvements generalize across model scales.
To validate our method, we construct a benchmark of 
%1,000
real-world customer service dialogues and evaluate simulators along three dimensions: session-level behavior, dialogue structure, and semantic consistency.
Experimental results show that TRACER significantly outperforms existing simulator approaches across all three dimensions, with especially large gains in decision-level behavioral consistency, a regime in which even the strongest proprietary LLMs exhibit large and erratic biases.
A key insight from our evaluation is that \textbf{stylistic alignment alone does not guarantee decision-level behavioral consistency}. 
Notably, a human-centered Turing test reveals that \textbf{TRACER is virtually indistinguishable from real users, whereas frontier LLMs are identified as machines in over 98\% of cases}. Furthermore, TRACER demonstrates strong generalization capabilities, consistently outperforming strongest baseline methods even in unseen scenarios.
%A human-centered Turing test corroborates this gap: our simulator is nearly indistinguishable from real users, while frontier LLMs are detected in over 98\% of cases.
%Ablation studies confirm that RL, trajectory-level reward, and turn-level credit assignment each contribute complementary gains that generalize across model scales.

% 【第5段：user simulator作为动态bench】
Furthermore, leveraging this high-fidelity user simulator, we introduce the Dynamic Marketing Benchmark, a user-centric suite evaluating LLMs as conversational marketing agents via multi-turn interactions with simulated users of diverse demographics. 
Unlike prior protocols that focus solely on response quality, DM-Bench jointly measures persuasion effectiveness and response quality, enabling a holistic view of agent capability. 
Benchmarking mainstream LLMs reveals a striking misalignment: top response quality does not guarantee high conversion in complex interactions.
%indicating that response quality alone fails to capture LLMs’ persuasion effectiveness 
% 【第6段：主要贡献】
% 本文的主要贡献包括：
% 1. 提出了一种基于真实用户数据驱动的用户模拟器框架 XXX，从语言与行为两个层面对齐真实用户；
% 2. 设计了一个面向多轮对话强化学习的训练框架，针对多轮交互中的奖励稀疏与信用分配问题，提出了轨迹级过程奖励建模与多轮优势分配策略，显著提升了训练稳定性与行为一致性

%\begin{itemize}
%\item 
%We propose \OurMethod, a novel multi-turn user simulator framework driven by real human interaction data. Going beyond the limitations of static persona prompting, \OurMethod~aligns simulated responses with real human distributions at both the linguistic-style level and the underlying decision-making level.
%方法，结论，动态benchmark
We summarize our contributions as follows:
1) We propose \OurMethod, a multi-turn user simulator aligned with real users at both linguistic and decision-making levels. It is trained in two stages: supervised fine-tuning followed by trajectory-aligned RL, which uses hierarchical rewards and trajectory-level advantage modulation to address reward coarseness and credit-assignment bias.
2) Experimental results show that \OurMethod{} outperforms strong proprietary baselines in session-level behavior, dialogue structure, and semantic consistency, and generalizes robustly to unseen scenarios. It passes a human-centered Turing test, with frontier LLMs detected over 98\% of the time.
3) Built on \OurMethod, we further develop a dynamic marketing  benchmark grounded in real user interactions, jointly measuring persuasion effectiveness and response quality.


%\end{itemize}

==> latex/4_method.tex <==
\section{\OurMethod}
\label{method}
% 主图
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.96\linewidth]{figure/main_v7.png}
  \caption{The \OurMethod{} framework: two-stage alignment of a user simulator along linguistic-style consistency and behavioral consistency rewards and trajectory-aligned credit assignment.}
  \label{fig:main}
\end{figure}

% 从人类交互轨迹中学习，需要在不同对话节奏之间建立对应关系，并确定由此得到的偏差应如何指导策略更新。
% \OurMethod 通过共享的轨迹对齐将这两项操作联系起来。
% 对齐同时提供用于评价完整交互的整体代价，以及用于调整逐轮更新的局部偏差。
% 下面先构造这些信号，再说明它们如何进入行为优化。
Learning from human interaction trajectories requires establishing correspondence across different conversational paces and deciding how the resulting deviations should guide policy updates. \OurMethod{} connects these two operations through a shared trajectory alignment. The alignment provides an overall cost for evaluating a completed interaction and local deviations for adjusting its turn-level updates. We first construct these signals, then describe how they enter behavioral optimization.

% 两阶段框架如图 \ref{fig:main} 所示。
% 按照第 3 节的定义，模拟器根据用户信息和交互历史生成解释、意图分数和用户回复。
% 第一阶段使用真实对话及其派生标注进行监督微调，初始化这些输出。
% 在第二阶段，模拟器与客服代理交互，生成用于多轮强化学习的完整轨迹。
% 这些轨迹依据关联的人类参考进行评分。
% 参考意图分数是用户状态的标注代理，为生成轨迹提供经验监督。
The two-stage framework is illustrated in Figure~\ref{fig:main}. Following the formulation in Section~3, the simulator generates a rationale, an intent score, and a user reply conditioned on the user information and interaction history. \textbf{Stage~1} uses supervised fine-tuning on real dialogues and their derived annotations to initialize these outputs. In \textbf{Stage~2}, the simulator interacts with a customer-service agent to generate complete trajectories for multi-turn reinforcement learning. These trajectories are scored against their associated human references. The reference intent scores are annotated proxies for user states and serve as empirical supervision for the generated trajectories.

% 行为轨迹的时间对齐
\subsection{Temporal Alignment of Behavioral Trajectories}
\label{sec:\OurMethod{}-alignment}

% 处理对话节奏差异。
\paragraph{Accounting for conversational pacing.}

% 相似的行为变化可能以不同节奏展开，使相同轮次编号之间的直接比较混淆时间偏移与行为偏差。
% 我们使用动态时间规整（DTW）建立保持顺序的对应关系，允许局部的一对多和多对一匹配。
Similar behavioral progressions may unfold at different paces, causing equal-index comparisons to confound temporal shifts with behavioral deviations. We use dynamic time warping (DTW; \citealp{dtw1,dtw2}) to establish an order-preserving correspondence that allows local one-to-many and many-to-one matches.

% 令 $z_{1:T}$ 和 $\hat z_{1:T^*}$ 分别表示参考与生成意图序列。
% 我们以状态的绝对差为局部代价，并沿最优对齐路径累积该代价：
Let $z_{1:T}$ and $\hat z_{1:T^*}$ denote the reference and generated intent sequences. We use the absolute state difference as the local cost and minimize its accumulation along the alignment path:
\begin{equation}
d(\hat z_i,z_j)=|\hat z_i-z_j|,
\label{eq:\OurMethod{}-local-cost}
\end{equation}
\begin{equation}
D_{\mathrm{DTW}}(\hat z_{1:T^*},z_{1:T})
=\min_{P}\sum_{(i,j)\in P}d(\hat z_i,z_j),
\label{eq:\OurMethod{}-dtw-cost}
\end{equation}
% 其中，$P$ 遍历满足边界、单调性和步长约束的对齐路径，在保持轮次顺序的同时允许局部时间伸缩。
% 动态规划得到最优代价及对应路径 $P^*$，分别用于整体轨迹评价与逐轮偏差提取；计算细节见附录 I。
where $P$ ranges over paths satisfying boundary, monotonicity, and step-size constraints, preserving turn order while allowing local temporal stretching. Dynamic programming yields the optimal cost and a corresponding path $P^*$ for trajectory-level evaluation and turn-level deviation extraction, respectively. Computational details are provided in Appendix~I.

% 提取整体与局部偏差。
\paragraph{Recovering global and local deviations.}
% 令 $P^*=((i_1,j_1),\ldots,(i_K,j_K))$ 表示一条最优对齐路径。
% 公式~\eqref{eq:\OurMethod{}-dtw-cost} 的累计代价汇总整体状态不匹配。
% 为保留其时间结构，我们还收集与每个生成轮次 $i$ 对齐的参考位置：
Let $P^*=((i_1,j_1),\ldots,(i_K,j_K))$ denote an optimal alignment path. The cumulative cost in Eq.~\eqref{eq:\OurMethod{}-dtw-cost} summarizes the overall state mismatch. To retain its temporal structure, we also collect the reference positions aligned with each generated turn $i$:
\begin{equation}
\begin{aligned}
A_i&=\{j_k\mid(i_k,j_k)\in P^*,\ i_k=i\},\\
d_i&=\frac{1}{|A_i|}\sum_{j\in A_i}|\hat z_i-z_j|.
\end{aligned}
\label{eq:\OurMethod{}-turn-deviation}
\end{equation}
% 当一个生成轮次匹配到多个参考位置时，在 $A_i$ 上取均值可为该轮得到一个局部偏差。
% 这两个量保留同一次对齐中的不同信息：$D_{\mathrm{DTW}}$ 衡量累计不匹配，$d_i$ 则给出各生成轮次的偏差大小。
% 前者用于构造轨迹奖励，后者用于调制不同轮次的策略更新。
Averaging over $A_i$ gives one local deviation per generated turn when that turn is matched to multiple reference positions. These two quantities preserve different information from the same alignment: $D_{\mathrm{DTW}}$ measures aggregate mismatch, whereas $d_i$ identifies its magnitude at each generated turn. We use the former to construct a trajectory reward and the latter to modulate policy updates across turns.

% 对齐引导的行为优化
\subsection{Alignment-Guided Behavioral Optimization}
\label{sec:\OurMethod{}-optimization}
% Compatibility with the reward-subsection reference in the original source.
\label{sec:hierarchical_reward}

% 评价完整交互。
\paragraph{Evaluating complete interactions.}
% 我们结合终态结果一致性、轨迹对齐和输出格式有效性。
% 终态奖励比较参考交互与生成交互的最终意图状态：
We combine terminal-outcome agreement, trajectory alignment, and output-format validity. The terminal reward compares the final intent states of the reference and generated interactions:
\begin{equation}
R_{\mathrm{final}}=\mathbb{I}(z_T=\hat z_{T^*}),
\label{eq:\OurMethod{}-final-reward}
\end{equation}
% 其中，$\mathbb{I}(\cdot)$ 是指示函数。
% 该项提供结果监督，而轨迹奖励进一步约束中间状态序列：
where $\mathbb{I}(\cdot)$ is the indicator function. This supplies outcome supervision, while the trajectory reward additionally constrains the intermediate state sequence:
\begin{equation}
R_{\mathrm{traj}}=
\exp\!\left(
-\alpha\cdot
\frac{D_{\mathrm{DTW}}(\hat z_{1:T^*},z_{1:T})+\beta|T^*-T|}{T}
\right)\cdot\eta.
\label{eq:\OurMethod{}-trajectory-reward}
\end{equation}
% 对齐代价衡量灵活时间对应关系下的状态偏差。
% 长度项单独惩罚轮数差异，以参考长度 $T$ 归一化则减弱代价对会话长度的依赖。
% 因此，允许局部灵活对齐并不意味着取消对整体交互长度的约束。
% 如附录 I 所述，当参考轨迹具有明显变化时，系数 $\eta\in(0,1]$ 对退化为近乎恒定状态的生成轨迹进行折扣。
The alignment cost measures state deviation under flexible temporal correspondence. The length term separately penalizes discrepancies in the number of turns, and normalization by the reference length $T$ reduces dependence on session length. Thus, flexible local alignment does not remove the constraint on overall interaction length. The coefficient $\eta\in(0,1]$ discounts degenerate, nearly constant generated trajectories when the reference exhibits substantial variation, as described in Appendix~I.

% 对于输出有效性，令 $r_t^{\mathrm{fmt}}\in\{0,1\}$ 表示第 $t$ 轮是否满足规定的结构格式和基本字段一致性检查。
% 格式奖励和总奖励为：
For output validity, let $r_t^{\mathrm{fmt}}\in\{0,1\}$ indicate whether turn $t$ satisfies the prescribed schema and basic field-consistency checks. The format reward and total reward are
\begin{equation}
R_{\mathrm{fmt}}=\frac{1}{T^*}\sum_{t=1}^{T^*}r_t^{\mathrm{fmt}},
\label{eq:\OurMethod{}-format-reward}
\end{equation}
\begin{equation}
R_{\mathrm{total}}
=\lambda_1R_{\mathrm{fmt}}+\lambda_2R_{\mathrm{final}}+\lambda_3R_{\mathrm{traj}},
\label{eq:\OurMethod{}-total-reward}
\end{equation}
% 其中，$\lambda_{1,2,3}$ 控制三个组成部分的贡献。
where $\lambda_{1,2,3}$ control the contributions of the three components.

% 在更新中保留时间信息。
\paragraph{Retaining temporal information in the update.}
% 虽然 $R_{\mathrm{total}}$ 使用了中间状态，但它仍然只为每次完整交互赋予一个标量。
% 获得相近奖励的轨迹，可能在不同位置或不同持续时段出现偏差。
% 将单一会话级优势广播到所有轮次，无法区分这些模式。
% 因此，我们保留公式~\eqref{eq:\OurMethod{}-turn-deviation} 的局部偏差，用它调整整体反馈的应用方式。
Although $R_{\mathrm{total}}$ incorporates intermediate states, it still assigns one scalar to each completed interaction. Trajectories with similar rewards can exhibit deviations at different positions or over different durations. Broadcasting a single session-level advantage across all turns does not distinguish these patterns. We therefore retain the local deviations from Eq.~\eqref{eq:\OurMethod{}-turn-deviation} and use them to adjust how the global feedback is applied.

% 令 $A_{\mathrm{traj}}$ 表示使用 GRPO（Shao 等，2024）根据交互采样奖励计算的标准化组相对优势。
% 对于生成轮次 $t$，我们汇总当前及后续的对齐偏差：
Let $A_{\mathrm{traj}}$ denote the standardized group-relative advantage computed from rollout rewards using GRPO \citep{shao2024deepseekmath} . For generated turn $t$, we summarize the current and subsequent alignment deviations by
\begin{equation}
c_t=\sum_{k=0}^{T^*-t}\rho^k\cdot d_{t+k},
\label{eq:\OurMethod{}-cumulative-deviation}
\end{equation}
% 其中，$\rho\in[0,1]$ 控制更远处偏差的影响。
% 与孤立的局部不匹配相比，$c_t$ 还反映偏差是否在后续轨迹中持续。
% 该量在交互采样完成后计算，提供与下游不匹配相关的信号，并不将最终结果因果归因于第 $t$ 轮。
where $\rho\in[0,1]$ controls the influence of more distant deviations. Unlike an isolated local mismatch, $c_t$ also reflects whether deviation persists in the subsequent trajectory. It is computed after the rollout and supplies a signal associated with downstream mismatch, rather than a causal attribution of the final outcome to turn $t$.

% 逐轮优势调制。
\paragraph{Turn-level advantage modulation.}
% 我们保留轨迹级优势作为整体学习信号，并在各轮调制其强度：
We preserve the trajectory-level advantage as the global learning signal and modulate its strength across turns:
\begin{equation}
\begin{aligned}
\widetilde A_t=w_t\cdot A_{\mathrm{traj}},\quad\quad
w_t=1-\lambda_{\mathrm{adv}}\cdot\operatorname{sign}(A_{\mathrm{traj}})
\cdot\tanh(\gamma c_t).
\end{aligned}
\label{eq:\OurMethod{}-advantage-modulation}
\end{equation}
% 其中，$\lambda_{\mathrm{adv}}\in[0,1]$ 控制调制幅度，$\gamma$ 控制对偏差的敏感程度。
% 当 $A_{\mathrm{traj}}>0$ 时，更大的 $c_t$ 会降低正向更新权重；当 $A_{\mathrm{traj}}<0$ 时，它会增大负向更新的幅度。
% 因此，与符号相关的因子将采样交互的整体质量与其时间偏差模式结合起来。
% 有界变换保留轨迹级优势的方向。
% 令 $\lambda_{\mathrm{adv}}=0$ 即恢复在各轮统一应用会话级优势；$c_t=0$ 的轮次保留单位权重。
Here, $\lambda_{\mathrm{adv}}\in[0,1]$ controls the modulation magnitude and $\gamma$ controls sensitivity to deviation. For $A_{\mathrm{traj}}>0$, a larger $c_t$ reduces the positive update weight; for $A_{\mathrm{traj}}<0$, it increases the magnitude of the negative update. The sign-dependent factor therefore combines the overall quality of the sampled interaction with its temporal deviation pattern. The bounded transformation preserves the direction of the trajectory-level advantage. Setting $\lambda_{\mathrm{adv}}=0$ recovers uniform application of the session-level advantage, and turns with $c_t=0$ retain unit weight.



==> latex/4_method_old.tex <==
\section{\OurMethod}
\label{method}
% 主图
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.96\linewidth]{figure/main_v7.png}
  \caption{The TRACER framework: two-stage alignment of a user simulator along linguistic-style consistency and behavioral consistency rewards and trajectory-aligned credit assignment.}
  \label{fig:main}
\end{figure}



% motivation 现有用户模拟方法大多侧重于学习与真实用户相似的表层语言风格，但在多轮交互场景下，决定模拟真实性的并不只是单轮回复是否自然，更在于用户模拟器是否遵循与真实用户一致的行为逻辑。这种行为逻辑不仅体现在最终意图状态的一致性上，也体现在整个交互过程中的动态一致性，包括意图状态的演化是否合理、交互节奏与轮次分布是否与真实模式相近。如果单纯依赖最终意图状态监督或者局部语言拟合，难以充分约束模拟器学习真实的多轮决策机制。同时，某一轮的局部决策偏差会进一步传导并影响后续多轮行为，而传统的强化学习优化通常以轨迹级回报作为主要监督，并默认同一条 session 内各轮动作共享近似均匀的训练信号，因而难以准确区分哪些局部决策真正导致了后续轨迹偏移与最终结果不一致。
% 因此，强化学习阶段需要解决两个关键问题：
% ● 如何构造能够刻画多轮行为一致性与轨迹合理性的行为信号；
% ● 如何在多轮轨迹上进行细粒度的优势分配，从而避免将session级别的反馈简单而均匀地施加到所有轮次，削弱对关键决策位置的有效学习。
%We propose \textbf{TRACER}, a two-stage framework that aligns a user simulator with real users along both \emph{linguistic-style} and \emph{behavioral consistency}. The overall pipeline is illustrated in Figure~\ref{fig:main}. In \textbf{Stage~1}, we perform supervised fine-tuning on real user dialogues to ground the simulator in user-like linguistic style and to initialize intent states inferred from observed user actions, providing a starting point for subsequent policy optimization. In \textbf{Stage~2}, we further align the simulator through RL with a hierarchical reward that jointly captures outcome-level and trajectory-level behavioral consistency, together with a trajectory-aligned advantage modulation that concentrates session-level feedback on the turns that actually drive trajectory drift.

%\paragraph{Motivation.}
Existing user simulators mainly align with real users in surface linguistic style. In multi-turn interactions, however, simulation fidelity depends more on whether the simulator follows a \emph{behavioral logic} consistent with real users, both in its terminal behavior and in the evolution of latent intents along the trajectory.
Neither terminal supervision nor local language
fitting captures such multi-turn decision dynamics, and local decision errors
further compound across turns. Aligning a simulator at the behavioral level through reinforcement learning therefore raises two challenges:
%The RL stage must therefore address two challenges: (1) constructing reward signals that capture multi-turn behavioral consistency and trajectory plausibility, and (2) performing fine-grained credit assignment so that session-level feedback is concentrated on critical decision points rather than uniformly diluted across all turns.
%Achieving behavioral consistency through reinforcement learning therefore raises two challenges:
\textbf{(1) Reward design beyond terminal outcomes.} A single session-level signal is too coarse to constrain how a trajectory unfolds; the reward must jointly capture outcome-level consistency and trajectory plausibility against real sessions.
\textbf{(2) Trajectory-aligned credit assignment.} Since turns contribute unequally to behavioral consistency, broadcasting
session-level feedback uniformly biases learning away from the pivotal decision
steps; credit must instead be re-weighted by each turn's contribution to session-level consistency.

To this end, we propose \textbf{TRACER}, a two-stage framework (Figure~\ref{fig:main}). \textbf{Stage 1} performs SFT on real dialogues to acquire user-like linguistic style and initialize latent intent states. \textbf{Stage 2} aligns behavior via RL with a hierarchical reward combining outcome- and trajectory-level consistency, and a trajectory-aligned advantage modulation. 
%These two challenges directly motivate the hierarchical reward and trajectory-aligned advantage modulation in TRACER.
%Existing user simulation methods primarily learn surface-level linguistic styles that mimic real users. But in multi-turn interactions, simulation fidelity hinges not on whether individual responses appear natural, but on whether the simulator follows \textbf{behavioral logic consistent} with real users. Such logic manifests in both the consistency of terminal intent states and the dynamic plausibility of the entire interaction trajectory—including whether intent evolution is coherent and whether turn-level pacing mirrors real-world patterns. Relying solely on terminal intent supervision or local language fitting is insufficient to capture authentic multi-turn decision-making mechanisms. Moreover, local decision errors at a given turn can propagate and compound across subsequent turns. Standard reinforcement learning approaches use trajectory-level returns as the primary signal and implicitly distribute credit approximately uniformly across turns within a session, making it difficult to pinpoint which local decisions actually cause trajectory drift and eventual outcome inconsistency.

%Existing user simulation methods mainly focus on learning surface-level linguistic styles that resemble those of real users. However, in multi-turn interaction scenarios, the realism of simulation is determined not merely by whether each individual response appears natural, but more importantly by whether the user simulator follows behavioral logic consistent with that of real users. Such behavioral logic is reflected not only in the consistency of terminal intent states, but also in the dynamic consistency of the entire interaction process, including whether the evolution of intent states is plausible and whether the interaction pacing and turn distribution resemble real-world patterns. If one relies solely on terminal intent supervision or local language fitting, it is difficult to adequately constrain the simulator to learn authentic multi-turn decision-making mechanisms. Moreover, local decision errors at a given turn may propagate and influence subsequent behaviors across multiple turns. Conventional reinforcement learning methods typically use trajectory-level returns as the primary supervision signal and implicitly assume that actions within the same session receive approximately uniform training signals, making it difficult to accurately identify which local decisions truly cause subsequent trajectory drift and eventual inconsistency in outcomes.


% 3.1 分层奖励设计
\subsection{Hierarchical Reward Design}
\label{sec:hierarchical_reward}
% 3.1.1 最终意图状态一致性奖励
\paragraph{Terminal Intent State Consistency Reward.}
% 最终意图状态z_T和\hat{z}_{T^*}反映了用户在交互时达到正向或者负向终止状态。基于此，我们首先引入最终意图状态一致性奖励，从结果层面对模拟轨迹施加约束，鼓励模型在会话结束时到达与真实用户一致的终局状态。具体地，该奖励定义为
% R_{final} = \mathbb{I} (z_T=\hat{z}_{T^*}) 
% 相比仅关注局部语言表面相似性，最终意图状态一致性奖励直接约束了模拟器是否在整段多轮交互后到达与真实用户一致的结果层状态，因此能够给行为策略学习提供清晰且语义明确的全局监督信号。
The terminal intent states $z_T$ reflects whether the user reaches a positive or negative terminal state during the interaction. Based on this, we first introduce a terminal intent state consistency reward to constrain the simulated trajectory at the outcome level, encouraging the simulator to reach the same terminal state as the real user. Specifically, this reward is defined as
\begin{equation}
R_{\mathrm{final}} = \mathbb{I}(z_T = \hat{z}_{T^*})
\end{equation}
Compared with rewards that focus only on local linguistic surface similarity, the terminal intent state consistency reward directly constrains whether the simulator reaches the same outcome-level state as the real user after the entire multi-turn interaction, thereby providing a clear and semantically meaningful global supervision signal for behavioral policy learning.


% 3.1.2 基于DTW的轨迹合理性奖励
% 然而，终局状态一致性不足以完整刻画多轮交互的行为逻辑：到达相同终局状态的两条轨迹，其中间阶段的状态演化路径与推进节奏可能存在显著差异。为此，我们在终局奖励之外引入轨迹合理性奖励，从过程层面约束模拟轨迹与真实轨迹的动态一致性。
% 由于真实与模拟轨迹在轮次数量、对话推进速度等上存在固有差异，严格的逐轮对齐对合理的时序伸缩缺乏鲁棒性。因此，我们采用Dynamic Time Warping（DTW）进行非线性时序对齐。设真实交互的意图序列为z_{1:T},模拟器生成的意图轨迹为\hat{z}_{1:T^*}，其中T和T^*分别为对应轨迹的轮次数。轨迹合理性奖励定义为：
% R_{traj} = exp (-\alpha \cdot \frac{D_{DTW}(\hat{z}_{1:T^*},z_{1:T})+\beta|T^*-T|}{T})\cdot \eta 
% 该奖励由三个组件协同构成：(1) D_{DTW}(z_{1:T},\hat{z}_{1:T^*})为DTW最优对齐代价，刻画意图演化路径的整体偏差（DTW的详细定义参见附录X）；(2)\beta|T^*-T|为轮次长度偏差惩罚，约束模拟轨迹的轮次数量不过度偏离真实轨迹；(3) \eta\in(0,1]
% 为平坦惩罚系数。我们观察到，仅依赖DTW与长度约束，模拟器倾向于生成近似恒定的意图序列以规避路径偏差惩罚。为抑制这一退化行为，当真实轨迹存在显著的意图状态变化而模拟轨迹长期停留于单一意图值时，\eta取小于1的折扣值。分母T对偏差进行长度归一化，使奖励在不同长度的轨迹间具有可比性。\alpha与\beta分别控制路径偏差与长度偏差的敏感程度。
% 直观地，R_{traj}在模拟轨迹的意图演化路径与真实轨迹高度吻合、轮次数量接近且意图变化模式一致时取得较高值。

\paragraph{DTW-based Trajectory Alignment Reward.}
\label{method:dtw_based_reward}
While terminal-state consistency ensures outcome alignment, it 
overlooks the behavioral dynamics of multi-turn interactions: 
two trajectories may reach the same conclusion via distinct 
intermediate transitions or paces. To enforce process-level 
consistency, we introduce a trajectory alignment reward that 
constrains the simulator's intent evolution to follow real 
interaction logic.

Drawing inspiration from speech signal processing, where Dynamic Time Warping (DTW) is the standard for measuring similarity between two sequences with varying speeds or temporal shifts~\citep{dtw1,dtw2}, we adapt DTW to dialogue intent sequences. This allows for a robust comparison that is invariant to \emph{temporal stretching}—common in dialogue when a simulator or user takes more/fewer turns to express the same intent. Let $z_{1:T}$ denote the intent sequence of the real interaction, and let $\hat{z}_{1:T^*}$ denote the intent trajectory generated by the simulator. The trajectory 
reward is
\begin{equation}
    R_{\mathrm{traj}} =\exp\left(-\alpha \cdot\frac{D_{\mathrm{DTW}}(\hat{z}_{1:T^*},z_{1:T}) + \beta |T^* - T|}{T}\right)\cdot \eta
\label{eq:dtw_trajectory_reward}
\end{equation}
which couples three components: 
(1) \textbf{path deviation}, $D_{\mathrm{DTW}}$, the optimal DTW 
alignment cost between intent paths (see 
Appendix~\ref{appendix:dtw_alignment}); 
(2) a \textbf{length penalty} $\beta|T^*-T|$ that discourages 
overly short or long trajectories; and
(3) a \textbf{diversity coefficient} $\eta\!\in\!(0,1]$, 
computed from the intent distribution of $\hat{z}$, which 
penalizes degenerate trajectories that repeat a single intent 
to trivially minimize the DTW cost.
Normalizing by $T$ ensures comparability across trajectory 
lengths.
%, while $\alpha$ and $\beta$ control the sensitivity to path and length deviations
%Intuitively, $R_{\mathrm{traj}}$ is higher when the simulated trajectory closely follows the real intent evolution, matches the number of turns, and maintains similar patterns of intent variation.
% 3.1.3 综合奖励设计
\paragraph{Overall Reward Formulation.}
% 前述两类奖励分别从结果层面和过程层面对模拟轨迹进行约束，但仅依赖session级监督仍不足以保证模型输出的结构合法性。为此，我们进一步引入格式奖励R_{fmt}，用于约束每轮输出满足预定义的结构化格式及基本字段一致性。记第t轮格式得分为r_t^{fmt}\in\{0,1\}，则有
% R_{fmt} = \frac{1}{T^*}\sum_{t=1}^{T^*}r_{t}^{fmt}
% 最终，整体奖励定义为
% R_{total}=\lambda_1R_{fmt}+\lambda_2R_{final}+\lambda_3R_{traj}
% 其中\lambda_1,\lambda_2,\lambda_3为权重系数。该分层奖励设计同时兼顾输出合法性、终局状态一致性与中间轨迹合理性，从而为多轮用户模拟提供更稳定、细粒度且语义明确的训练信号。
While the two rewards above supervise the simulated trajectory at the outcome and process levels, neither enforces the structural validity of per-turn outputs.  We thus introduce a format reward $R_{\mathrm{fmt}}$, which checks whether each turn conforms to a predefined schema and maintains basic field consistency. Let the format score at turn $t$ be $r_t^{\mathrm{fmt}} \in \{0,1\}$, then
\begin{equation}
    R_{\mathrm{fmt}} = \frac{1}{T^*}\sum_{t=1}^{T^*} r_t^{\mathrm{fmt}}
\end{equation}
The overall reward combines the three components:
\begin{equation}
    R_{\mathrm{total}} = \lambda_1 R_{\mathrm{fmt}} + \lambda_2 R_{\mathrm{final}} + \lambda_3 R_{\mathrm{traj}}
\label{eq:overall_reward}
\end{equation}
%where $\lambda_1$, $\lambda_2$, and $\lambda_3$ are weighting coefficients. This hierarchical reward design jointly considers output validity, terminal-state consistency, and intermediate trajectory plausibility, thereby providing more stable, fine-grained, and semantically meaningful training signals for multi-turn user simulation.
where $\lambda_{1,2,3}$ are weighting coefficients. This design jointly enforces output validity, terminal-state consistency, and trajectory plausibility, yielding more stable and fine-grained signals for multi-turn user simulation.

% 3.2 细粒度优势分配
\subsection{Trajectory-aligned Advantage Modulation}
\label{method:advantage_modulation}
% 尽管第 4.1 节的分层奖励能够从终局结果与轨迹过程两个层面对模拟轨迹进行评估，session级反馈仍不足以有效优化多轮用户模拟。核心原因在于，多轮交互中的行为偏差具有延迟传导特征：早期轮次的微小偏移可能经后续轮次逐步累积，而后期的显性错误往往只是前序偏差的结果。若将session级advantage均匀施加到所有轮次（即GRPO在多轮场景中的常见做法），模型将难以识别真正驱动轨迹偏移的关键决策位置。
% 为此，我们提出细粒度优势分配机制：在保留轨迹级advantage作为全局优化方向的前提下，依据各轮对后续轨迹偏差的潜在责任，对session内不同轮次的优势进行重分配。轨迹级advantage决定整条样本应被鼓励或抑制，而轮次级偏差信号进一步决定样本内部各位置的学习强度。换言之，我们并不改变原有强化学习目标，而是在其基础上引入面向多轮场景的credit assignment修正。
% The hierarchical reward in Section~\ref{sec:hierarchical_reward} still
% collapses into a session-level scalar, which is insufficient for multi-turn
% optimization. 
% Behavioral deviations propagate with delay: subtle drifts in early
% turns accumulate over subsequent ones, so the turns where errors become visible
% are often mere consequences of earlier, causal decisions. Standard
% GRPO-style\citep{shao2024deepseekmath} training broadcasts the session-level advantage uniformly, collapsing causal and consequential turns into a single signal, and thus obscuring where drift originates.
%conflating these causal and consequential turns and 
%The core reason is that behavioral deviations in multi-turn interaction exhibit a delayed propagation effect: subtle deviations in early turns can accumulate over subsequent turns, and seemingly explicit errors in later turns are often mere consequences of earlier drift. Under the common GRPO-style practice of broadcasting the session-level advantage uniformly to all turns, the model struggles to localize the critical decision points that actually trigger trajectory drift.

%To address this, we propose a fine-grained advantage allocation mechanism. While preserving the trajectory-level advantage as the global optimization direction, we redistribute it across turns according to each turn's estimated responsibility for downstream deviation. Intuitively, the trajectory-level advantage decides whether a sample should be reinforced or suppressed as a whole, while a turn-level deviation signal modulates the learning intensity at each position within the sample. Rather than altering the underlying RL objective, our method introduces a credit assignment correction tailored to multi-turn settings on top of it. 
% We address this with a trajectory-aligned advantage modulation that keeps the trajectory-level advantage as the global signal, but reweights it across turns according to their contribution to session-level
% inconsistency, measured by the per-turn discrepancy in intent score. 
% This can be viewed as a turn-level reweighting of the trajectory-level advantage, leaving the RL objective unchanged.
%; the formal definition of $w_t$ is given next.
The rewards in Section~\ref{sec:hierarchical_reward} collapse into a session-level scalar, which is insufficient for multi-turn optimization. Standard GRPO-style~\citep{shao2024deepseekmath} training broadcasts this session-level advantage uniformly across all turns, collapsing them into a single signal and providing no turn-specific information about where alignment deviations occur. We address this with a trajectory-aligned advantage modulation that retains the trajectory-level advantage as the global signal, but reweights it across turns according to the temporal pattern of alignment deviations, measured by the per-turn discrepancy in intent score. This can be viewed as a turn-level reweighting of the trajectory-level advantage: the update weight varies across turns, while the session-level signal remains the basis for reinforcing or suppressing a sampled trajectory
% 未来偏差得分
\paragraph{Cumulative Alignment Deviation.}
% 对于生成轨迹中的第t轮，定义其未来偏差得分c_t
% c_t= \sum_{k=0}^{T^*-t} \rho^k\cdot d_{t+k}
% 其中，d_{t+k}表示DTW对齐后第t+k轮的局部偏差度量（见附录X），\rho \in (0,1]为折扣因子。c_t刻画从第t轮起后续轨迹的累计偏差。
For turn $t$ in a generated trajectory, we define its cumulative future deviation $c_t$ as
\begin{equation}
    c_t = \sum_{k=0}^{T^*-t} \rho^k \cdot d_{t+k}
\label{eq:future_deviation_score}
\end{equation}
where $d_{t+k}$ denotes the local deviation measure at turn $t+k$ after DTW alignment (see Appendix~\ref{appendix:dtw_alignment}), and $\rho \in [0,1]$ controls
how far downstream deviations influence the credit of turn $t$. Intuitively, $c_t$ summarizes how much the trajectory drifts after
turn $t$, providing a per-turn signal of its causal contribution to
session-level inconsistency.

% 轮次级优势调制
\paragraph{Turn-level Advantage Modulation.}
% 基于c_t构造轮次级权重:
% w_t=1-\lambda \cdot \frac{A}{|A|+\epsilon}\cdot tanh (\eta\cdot c_t)
% 其中，A表示该session的轨迹级advantage (计算方式同GRPO)，\epsilon为数值稳定项，\lambda控制重新加权的幅度，\eta控制模型对偏差的敏感度。当A>0时，高c_t的轮次权重降低——尽管轨迹整体较优，但该轮之后伴随较大偏移，不应获得同等强度的正向强化；当A<0时，高c_t的轮次权重增大——该轮更可能与后续持续偏移相关，应承受更强的负向更新。
We use $c_t$ to reweight the trajectory-level advantage
$A_{\text{traj}}$ (the standardized group-relative advantage from GRPO)
into a turn-level advantage:
\begin{equation}
    \tilde{A}_t = w_t \cdot A_{\text{traj}}, \qquad
    w_t = 1 - \lambda_{\text{adv}} \cdot
          \mathrm{sign}(A_{\text{traj}}) \cdot
          \tanh(\gamma\, c_t),
\label{eq:advantage_modulation_weight}
\end{equation}
%where $A$ denotes the trajectory-level advantage of the session (computed in the same way as in GRPO), $\epsilon$ is a numerical stability term, $\lambda_{adv}$ controls the magnitude of reweighting, and $\gamma$ controls the model's sensitivity to deviation.
%When $A > 0$, turns with larger $c_t$ receive lower weights. This means that although the overall trajectory is relatively good, the turns followed by larger deviations should not receive equally strong positive reinforcement. In contrast, when $A < 0$, turns with larger $c_t$ receive higher weights, because such turns are more likely to be associated with persistent downstream deviation and should therefore undergo stronger negative updates.
where $\lambda_{\text{adv}} \in [0,1]$ controls the modulation magnitude
and $\gamma$ the sensitivity to deviation. The $\mathrm{sign}$ factor
flips the modulation direction with the trajectory's overall quality,
while $\tanh(\gamma c_t)\!\in\![0,1)$ keeps the reweighting bounded so
that $w_t$ stays close to unity and the trajectory-level signal is
modulated rather than overwritten. Concretely, turns with larger
 cumulative future deviation are down-weighted when reinforcing a good
trajectory ($A_{\text{traj}}{>}0$) and up-weighted when
suppressing a bad one ($A_{\text{traj}}{<}0$), so that updates
concentrate on the turns most responsible for drift.
This modifies only the per-turn advantage construction, leaving the
PPO-style clipped objective of GRPO unchanged.
% Token级广播
%\paragraph{Token-level Broadcasting.}
% 将轮次权重广播到对应的所有有效token。记第t轮第j个token的原始advantage为A_{t,j}，重分配后的advantage为：
% \tilde{A}_{t,j}=w_t\cdot A_{t,j}
% 这样，模型不仅学习这条轨迹整体质量，还能区分同一轨迹内各轮次的学习优先级。值得注意的是，本机制与基于价值函数的时序差分方法（如 GAE）在思路上有本质区别：我们并不依赖 critic 估计每个状态的长期价值，而是直接利用可观测的轨迹偏差信号进行后验的责任归因，从而规避了在用户模拟这一状态空间开放的场景中训练critic所面临的不稳定性。
%We broadcast the turn-level weight to all valid tokens in the corresponding turn. Let $A_{t,j}$ denote the original advantage of the $j$-th token at turn $t$, and let $\tilde{A}_{t,j}$ denote the reallocated advantage. Then
%\begin{equation}
%    \tilde{A}_{t,j} = w_t \cdot A_{t,j}
%\end{equation}

%In this way, the model learns not only the overall quality of a trajectory, but also the relative learning priority of different turns within the same trajectory. It is worth noting that this mechanism is fundamentally different from value-based temporal-difference methods such as GAE. We do not rely on a critic to estimate the long-term value of each state; instead, we directly use observable trajectory deviation signals for post hoc responsibility attribution. This design avoids the instability of critic training in user simulation, where the state space is highly open-ended.

==> latex/6_further_old.tex <==
\section{Application: Dynamic Marketing Benchmark}
\begin{figure}[htbp]
    \centering
    % === 1. 将左侧宽度提至 0.63，右侧 0.35，总计 0.98，剩下的 \hfill 只有极小间隙 ===
    %\vspace{-15pt}
    % --- 左侧区域 (a, b, c, d) ---
    \begin{minipage}[b]{0.58\textwidth}
        % --- 第一行：a 和 b ---
        \begin{center}
            % a/b/c/d 统一使用 0.49\linewidth 保证标题上下绝对对齐
            \begin{subfigure}[b]{0.46\linewidth}
                \centering
                % 将原本的 0.85 放大到 0.95 或 0.98，视觉留白会瞬间变少
                \includegraphics[width=0.95\linewidth]{figure/profile_personality_v2.png}
                \captionsetup{font=footnotesize}
                \caption{Personality}
                \label{fig:c}
            \end{subfigure}
            \hfill % 自动分配极小留白
            \begin{subfigure}[b]{0.49\linewidth}
                \centering
                \includegraphics[width=0.98\linewidth]
                {figure/profile_city_v2.png}
                \captionsetup{font=footnotesize}
                \caption{City Profile}
                \label{fig:b}
            \end{subfigure}
        \end{center}

        % --- 第二行：c 和 d ---
        \begin{center}
        \begin{subfigure}[b]{0.46\linewidth}
                \centering
                % 图片填满容器的大部分 (0.98)，减少内部留白
                \includegraphics[width=0.98\linewidth, height=2cm]{figure/profile_age_v2.png}
                \captionsetup{font=footnotesize}
                \caption{Demographic Profile} 
                \label{fig:a}
            \end{subfigure}
            \hspace{0.2em} 
            \begin{subfigure}[b]{0.48\linewidth}
                \centering
                \includegraphics[width=0.85\linewidth]
                {figure/profile_industry_v2.png}
                \captionsetup{font=footnotesize}
                \caption{Merchant Distribution}
                \label{fig:d}
            \end{subfigure}
        \end{center}
    \end{minipage}
    \hspace{0.1em}
    % --- 右侧区域 (e) ---
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=5.5cm]{figure/bench_v4.png}
        \captionsetup{font=footnotesize}
        \caption{LLM Performance as Customer Service Agents}
        \label{fig:e}
    \end{subfigure}

    \caption{Overview of DM-Bench: User Profiles, Merchant Distribution, and Model Performance.}
    \label{fig:total}
    \vspace{-0.9pt}
\end{figure}

Existing benchmarks for conversational persuasion and marketing dialogue are limited in two ways. They are largely static, relying on single-turn scoring or fixed transcript replay, and they are quality-oriented, focusing on surface-level properties such as fluency or perceived persuasiveness rather than downstream behavioral outcomes. As a result, they fail to evaluate whether an agent can adapt over multiple turns and ultimately drive conversion.
We address this gap with DM-Bench, an outcome-driven, user-centric dynamic benchmark built on the high-fidelity user simulator introduced.
%in Section~\ref{method}
%DM-Bench evaluates mainstream LLMs through multi-turn interactions with 734 heterogeneous simulated users, using conversion as the terminal outcome signal.

%To close this gap, we leverage the high-fidelity user simulator developed in Section~\ref{method} to construct DM-Bench, an outcome-driven, user-centric dynamic benchmark in which mainstream LLMs are evaluated against 1,000 heterogeneous simulated users over multi-turn dialogues, with conversion as the terminal signal.

\subsection{Benchmark Construction}
%DM-Bench is instantiated from the 793 sessions of CustomerService-Dialogue. Each instance is represented as a triplet $(\mathcal{U}, \mathcal{I}, \mathcal{M})$, corresponding to the user profile, initial user intent, and merchant context. Since the data source and split have been introduced in Section~\ref{xxx}, we omit repeated dataset details here.
%DM-Bench is instantiated from the 793 sessions of CustomerService-Dialogue. Each instance consists of two components: user profile information $\mathcal{U}$ and merchant information $\mathcal{M}$. The user profile contains the user's demographic attributes and initial intent, while the merchant information provides the business-side context available to the customer-service agent. Since the data source and construction protocol have been introduced in Section~\ref{xxx}, we omit repeated dataset details here.

DM-Bench is instantiated by sampling 734 sessions from CustomerService-Dialogue while preserving the empirical data distribution. Each instance contains two components: user profile information and merchant information. The user profile includes demographic attributes, and the initial intent, while the merchant information provides the business-side context. The distributions of user profiles and merchant industries are shown in Figure~\ref{fig:total}. Since the data source and construction protocol have been introduced in Section~\ref{sec:experimental}, we omit repeated dataset details here.
%Each instance in DM-Bench is defined by a triplet $(\mathcal{U}, \mathcal{I}, \mathcal{M})$, where $\mathcal{U}$ is a user persona, $\mathcal{I}$ the user's initial intent, and $\mathcal{M}$ the merchant context provided to the agent. We construct 1,000 user personas spanning differentiated attributes across four dimensions: demographics, consumption preferences, psychological traits (e.g., persuasion openness, decision style), and domain knowledge. Each dialogue proceeds between the evaluated LLM (acting as the marketing agent, conditioned on $\mathcal{M}$) and our user simulator (initialized with $\mathcal{U}$ and $\mathcal{I}$), for up to 15 turns, terminating early upon purchase, explicit disengagement, or natural conclusion.
%\paragraph{Evaluation Instances.} Each instance in DM-Bench is defined by a triplet $(\mathcal{U}, \mathcal{I}, \mathcal{M})$: a user persona $\mathcal{U}$, an initial intent $\mathcal{I}$, and a merchant context $\mathcal{M}$. We construct \#\#\# user personas with differentiated attributes across demographics, consumption preferences, psychological traits (e.g., persuasion openness, decision style), and domain knowledge. 
DM-Bench evaluates dialogue agents from both user-centered conversion outcomes and conventional response quality.  We report three complementary metrics.
\textbf{Conversion Rate (CR)} measures the proportion of sessions that end with conversion, as determined by the user simulator, and serves as the primary indicator of persuasion effectiveness. 
%\textbf{Conversion Turns (CT)} denotes the average number of dialogue turns among converted sessions. 
\textbf{Response Quality (RQ)} is an LLM-as-a-judge score following \citep{zhu2026evaluating}, which evaluates multi-turn responses in terms of accuracy, helpfulness, informativeness and empathy. 
%To mitigate self-preference bias, we use gpt-oss-120B\citep{openai2025gptoss120bgptoss20bmodel} as the judge.
\subsection{Results and Findings}
We report the results in Figure \ref{fig:total}, Table~\ref{tab:dm_bench_full_results} and Table~\ref{tab:cr_rq_spearman}, with the following conclusions: 
%First, response quality and conversion effectiveness are only weakly aligned. Across the seven models, the rank correlation between RQ and CR is small and non-significant (Spearman $\rho\approx0.21$, $n=7$), in sharp contrast with the intuition that better-sounding responses should yield better persuasion outcomes. 
\textbf{(1) Response quality is not a reliable proxy for conversion effectiveness.} Although RQ and CR show a moderate positive rank correlation across the seven models (Spearman $\rho = 0.57$, $p = 0.18$, $n=7$); for instance, Claude-4.5-Sonnet ranks highest on RQ but is surpassed on CR by DeepSeek-V3.2 and Qwen3-235B. This indicates that response-quality evaluation does not fully capture persuasion effectiveness.
\textbf{(2) Even frontier LLMs exhibit a substantial conversion ceiling.} Despite high response-quality scores, top models still fail to convert a large fraction of users, revealing limited adaptation to user intent and decision dynamics in multi-turn interactions.


%Two observations emerge. First, response quality and conversion effectiveness are not strongly aligned: Qwen2.5-7B attains a competitive RQ of 68.17 yet converts only 36.8\% of sessions, while Doubao-pro achieves the lowest RQ but a mid-tier CR. This corroborates the view that stylistic excellence does not directly translate into persuasion effectiveness—fluent, informative replies may still fail to drive user decisions. Second, stronger frontier models (DeepSeek, Claude, Gemini) lead on both axes but with non-trivial gaps in CR (0.51–0.56), indicating that persuading heterogeneous, skeptical users in multi-turn settings remains an open challenge even for state-of-the-art LLMs.
These findings show the value of DM-Bench as a user-centered, outcome-driven evaluation protocol: it reveals performance gaps that are largely invisible under quality-only benchmarks, especially the gap between generating good-sounding responses and generating decision-moving ones.
%\textbf{Overall performance.} Table 4 reports the main results.


%DM-Bench 的结果表明，当前的LLM虽然能够进行基本的营销对话，但在心智理论（检测隐性态度转变）、战略规划（连贯的多轮说服）和适应性沟通（针对不同用户群体进行定制）方面存在根本性的局限性。这些发现从两个方面补充了本文的主要贡献。诊断结果（例如，战略规划的关键作用、面对持怀疑态度的用户时遇到的困难）为改进基于LLM的智能体指明了具体方向，我们的模拟器可以作为训练环境，用于开发更复杂的对话策略。
%These findings validate that our user simulator enables a user-centric, outcome-driven evaluation that prior quality-only protocols overlook, and expose a key limitation of current LLMs: the gap between generating good-sounding responses and generating decision-moving ones.
